Benchmarking seismic phase associators: Insights from synthetic scenarios

Reliable seismicity catalogs are essential for seismology. Following phase picking, phase association groups arrivals into sets with consistent origins (i.e., events), determines event counts, and identifies outlier picks. To handle the substantial increase in the quantity of seismic phase picks from improved picking methods and larger deployments, several novel phase associators have recently been proposed. This study presents a detailed benchmark analysis of five seismic phase associators, including classical and machine learning-based approaches: PhaseLink, REAL, GaMMA, GENIE, and PyOcto. We use synthetic datasets mimicking real seismicity characteristics in crustal and subduction zone scenarios. We evaluate performance for different conditions, including low- and high-noise environments, out-of-network events, very high event rates, and variable station density. The results reveal notable differences in precision, recall, and computational efficiency. GENIE and PyOcto demonstrate robust performance, with almost perfect performance for most scenarios. Only for the most challenging conditions with high noise levels and event rates, performance drops but still maintains F1 scores above 0.8. PhaseLink's performance declines with noise and event density, particularly in subduction zones, dropping to near zero in the most complex cases. GaMMA outperforms PhaseLink but struggles with accuracy and scalability in high-noise, high-density scenarios. REAL performs reasonably but loses recall under extreme conditions. PyOcto and PhaseLink show the quickest runtimes for smaller-scale datasets, while REAL and GENIE are more than an order of magnitude slower for these cases. At the highest pick rates, GENIE's runtime disadvantage diminishes, matching PyOcto and scaling effectively. Our results can guide practitioners compiling seismicity catalogs and developers designing novel associators.

==> figures/versions_battle/versions_battle_california/associator_stats.tex <==
\begin{tabular}{rrlllll}
\hline
 Events &  Noise & Associator & Event\_Precision & Event\_Recall & Event\_F1\_Score & Runtime (s) \\
\hline
    100 &     30 &   GaMMA 0D &            0.98 &         1.00 &           0.99 &       13.27 \\
    100 &     30 &   GaMMA 1D &            1.00 &         1.00 &           1.00 &        9.89 \\
    100 &     30 &  PyOcto 0D &            1.00 &         1.00 &           1.00 &        1.98 \\
    100 &     30 &  PyOcto 1D &            1.00 &         1.00 &           1.00 &        2.71 \\
    100 &     30 &    REAL 0D &            1.00 &         0.98 &           0.99 &        9.46 \\
    100 &     30 &    REAL 1D &            1.00 &         0.98 &           0.99 &        6.90 \\
    100 &    100 &   GaMMA 0D &            0.98 &         0.98 &           0.98 &       19.97 \\
    100 &    100 &   GaMMA 1D &            1.00 &         0.99 &           0.99 &       13.22 \\
    100 &    100 &  PyOcto 0D &            1.00 &         0.98 &           0.99 &        3.46 \\
    100 &    100 &  PyOcto 1D &            1.00 &         0.98 &           0.99 &        3.42 \\
    100 &    100 &    REAL 0D &            1.00 &         0.98 &           0.99 &       31.51 \\
    100 &    100 &    REAL 1D &            1.00 &         0.98 &           0.99 &       20.48 \\
    100 &    300 &   GaMMA 0D &            0.98 &         0.99 &           0.99 &       22.73 \\
    100 &    300 &   GaMMA 1D &            0.99 &         0.99 &           0.99 &       18.56 \\
    100 &    300 &  PyOcto 0D &            1.00 &         0.99 &           0.99 &        8.89 \\
    100 &    300 &  PyOcto 1D &            1.00 &         0.99 &           0.99 &        5.84 \\
    100 &    300 &    REAL 0D &            1.00 &         0.99 &           0.99 &       75.32 \\
    100 &    300 &    REAL 1D &            1.00 &         0.99 &           0.99 &       58.76 \\
    500 &     30 &   GaMMA 0D &            0.98 &         0.99 &           0.99 &      118.46 \\
    500 &     30 &   GaMMA 1D &            0.99 &         0.99 &           0.99 &       46.43 \\
    500 &     30 &  PyOcto 0D &            0.99 &         0.96 &           0.98 &       24.42 \\
    500 &     30 &  PyOcto 1D &            1.00 &         0.97 &           0.98 &       19.02 \\
    500 &     30 &    REAL 0D &            1.00 &         0.93 &           0.96 &       48.30 \\
    500 &     30 &    REAL 1D &            1.00 &         0.93 &           0.97 &       38.62 \\
    500 &    100 &   GaMMA 0D &            0.99 &         1.00 &           0.99 &      164.97 \\
    500 &    100 &   GaMMA 1D &            1.00 &         1.00 &           1.00 &       67.81 \\
    500 &    100 &  PyOcto 0D &            0.99 &         0.98 &           0.99 &       11.66 \\
    500 &    100 &  PyOcto 1D &            1.00 &         0.98 &           0.99 &       10.95 \\
    500 &    100 &    REAL 0D &            0.99 &         0.93 &           0.96 &      145.26 \\
    500 &    100 &    REAL 1D &            1.00 &         0.93 &           0.96 &      109.86 \\
    500 &    300 &   GaMMA 0D &            0.79 &         0.99 &           0.88 &      393.30 \\
    500 &    300 &   GaMMA 1D &            0.79 &         0.99 &           0.88 &      150.07 \\
    500 &    300 &  PyOcto 0D &            0.99 &         0.98 &           0.98 &       40.73 \\
    500 &    300 &  PyOcto 1D &            1.00 &         0.98 &           0.99 &       21.26 \\
    500 &    300 &    REAL 0D &            0.98 &         0.93 &           0.96 &      419.16 \\
    500 &    300 &    REAL 1D &            0.94 &         0.94 &           0.94 &      322.31 \\
   2000 &     30 &   GaMMA 0D &            0.96 &         0.99 &           0.97 &     1321.14 \\
   2000 &     30 &   GaMMA 1D &            0.98 &         0.99 &           0.98 &      312.27 \\
   2000 &     30 &  PyOcto 0D &            0.98 &         0.92 &           0.95 &       71.05 \\
   2000 &     30 &  PyOcto 1D &            0.99 &         0.93 &           0.96 &       51.07 \\
   2000 &     30 &    REAL 0D &            0.99 &         0.78 &           0.87 &      239.90 \\
   2000 &     30 &    REAL 1D &            0.98 &         0.80 &           0.88 &      195.39 \\
   2000 &    100 &   GaMMA 0D &            0.57 &         0.96 &           0.71 &     4195.28 \\
   2000 &    100 &   GaMMA 1D &            0.57 &         0.96 &           0.71 &      900.20 \\
   2000 &    100 &  PyOcto 0D &            0.96 &         0.92 &           0.94 &      198.28 \\
   2000 &    100 &  PyOcto 1D &            0.99 &         0.92 &           0.95 &      136.43 \\
   2000 &    100 &    REAL 0D &            0.96 &         0.79 &           0.87 &      551.88 \\
   2000 &    100 &    REAL 1D &            0.92 &         0.81 &           0.86 &      506.13 \\
   2000 &    300 &  PyOcto 0D &            0.69 &         0.89 &           0.78 &     1323.13 \\
   2000 &    300 &  PyOcto 1D &            0.73 &         0.91 &           0.81 &     1170.82 \\
   2000 &    300 &    REAL 0D &            0.91 &         0.73 &           0.81 &     1985.60 \\
   2000 &    300 &    REAL 1D &            0.60 &         0.77 &           0.67 &     1680.00 \\
\hline
\end{tabular}

